Deformation theory of the blown-up Seiberg-Witten equation in dimension three

Associated with every quaternionic representation of a compact, connected Lie group there is a Seiberg-Witten equation in dimension three. The moduli spaces of solutions to these equations are typically non-compact. We construct Kuranishi models around boundary points of a partially compactified moduli space. The Haydys correspondence identifies such boundary points with Fueter sections - solutions of a non-linear Dirac equation - of the bundle of hyperk\"ahler quotients associated with the quaternionic representation. We discuss when such a Fueter section can be deformed to a solution of the Seiberg-Witten equation.

==> SeibergWittenEquation.tex <==
\section{Seiberg--Witten equations}
\label{Sec_SeibergWittenEquations}

Let $S$ and $G$ be as in \autoref{Sec_HyperkahlerQuotients} and let $H$ be a Lie group acting on $S$, preserving $\gamma$ and commuting with $G$.

Let $(M,g,\fs)$ be a spin $3$--manifold, $P$ a $G$--bundle on $M$, and $Q$ a $H$--bundle on $M$.

We have a canonical isomorphism
\begin{equation*}
  T^*M \iso \fs \times_{\Spin(3)} \Im \H
\end{equation*}
as \emph{oriented} Euclidean bundles.
(Here we declare where $(i,j,k)$ to be a positive basis of $\Im H$.)

\begin{definition}
  The \defined{spinor bundle} associated with $S$ is
  \begin{equation*}
    \fS := (\fs\times P \times Q)\times_{\Spin(3)\times G \times H} S;
  \end{equation*}
  and the \defined{Clifford multiplication} is denote by $\gamma\co T^*M \to \End(\fS)$.
\end{definition}

\begin{remark}[I think we don't need that remark, but I'll leave it in for the time being]
  With the above orientation convention, whenever $(e^1,e^2,e^3)$ is a orthonormal basis of $T^*_xM$, then
  \begin{equation*}
    \gamma(e^i)\gamma(e^j) = \epsilon_{ijk}\gamma(e^k).
  \end{equation*}
  We can extend the action of $T^*M$ on $S$ to $\Lambda^2T^*M$ by declaring that
  \begin{equation*}
    \gamma(e^i\wedge e^j)
    = \frac12[\gamma(e^i),\gamma(e^j)]
    = \sum_{k=1}^3 \epsilon_{ijk}\gamma(e^k).
  \end{equation*}
  Here $\epsilon_{ijk}$ is the totally anti-symmetric symbol.
  Since we also have
  \begin{equation*}
    *(e^i\wedge e^j) = \sum_{k=1}^3 \epsilon_{ijk} e^k \qandq
    ** = \id,
  \end{equation*}
  this means that $\gamma(*\alpha) = \gamma(\alpha)$.  
\end{remark}

The Levi--Civita connection induces a connection on $\fs$, which we can use together with $A$ and $B$ to differentiate sections of $\fS$:
$\Phi \in \Gamma(\fS) \mapsto \nabla_{AB} \Phi \in \Omega^1(M,\fS)$.
\begin{definition}
  The \defined{Dirac operator} is
  \begin{equation*}
    \slD_{AB} \Phi = \gamma(\nabla_{AB}\Phi).
  \end{equation*}
\end{definition}

Identifying $\fs \times_{\Spin(3)} \Im \H \iso T^*M \stackrel{*}{\iso} \Lambda^2 T^*M$, the map $\mu$ induces a quadratic map $\mu \co \Gamma(\fS) \to \Omega^2(M,\fg_P)$ (and or a linear map $\mu\co \Gamma(\fS)^{\otimes 2} \to \Omega^2(M,\fg_P)$).

\begin{definition}
  The \defined{Seiberg--Witten equation} associated with $(S,G\times H,\rho)$ is the equation
  \begin{equation}
    \label{Eq_SeibergWitten}
    \begin{split}
      \slD_{AB}\Phi 
      &= 0 \\
      F_A 
      &= \mu(\Phi).
    \end{split}
  \end{equation}
  for $(\Phi,A) \in \Gamma(\fS) \times \sA(P)$.
\end{definition}

\begin{definition}
  The \defined{Seiberg--Witten moduli space} is
  \begin{equation*}
    \fM 
    :=
    \set{
      (\Phi,A) \in \Gamma(\fS) \times \sA(P)
      :
      \eqref{Eq_SeibergWitten}
    } / \sG(P).
  \end{equation*}
\end{definition}

We can define a natural metric on $\fM$ and thus equip $\fM$ with a topology.
In the case of the usual Seiberg--Witten equation, $\fM$ is compact.
This will usally not hold for $(S, G \times H,\rho)$.
It is typically possible for $\Phi$ to be come very large.
To this end we blow-up the equation by replacing $\Phi$ with $\epsilon^{-1} \Phi$ with $\Abs{\Phi}_{L^2} = 1$.

\begin{definition}
  The \defined{blown-up Seiberg--Witten equation} associated with $(V,G)$ is the following p.d.e.~for $(\Phi,A,\epsilon) \in \Gamma(\fS) \times \sA(P) \times (0,\infty)$
  \begin{equation}
    \label{Eq_BlownUpSeibergWitten}
    \begin{split}
      \slD_{AB}\Phi 
      &=
        0 \\
      -\epsilon^{2}*F_A +  \mu(\Phi) 
      &= 0   \\
      \Abs{\Phi}_{L^2}
      &=
        1.
    \end{split}
  \end{equation}
\end{definition}

We can formally allow for $\epsilon = 0$.

This indicates that one can \emph{partially} compactify $\fM$ by including Fueter sections of $\fX$.
(By \cite{Taubes2012,Taubes2013,Haydys2014} we know that this is now quite enough.
One has to allow ``singular'' Fueter sections as well.
Since we don't understand those well, we can't deal with them here.)


\begin{definition}
  The \defined{partially compactified Seiberg--Witten moduli space} is
  \begin{equation*}
    \bar \fM 
    :=
    \set{
      (\Phi,A,\epsilon ) \in \Gamma(\fS) \times \sA(P) \times [0,\infty)
      :
      \eqref{Eq_BlownUpSeibergWitten}
    } / \sG(P).
  \end{equation*}
\end{definition}

Our aim will be to understand a neighbourhood of the $\epsilon = 0$ slice of $\bar\fM$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SeibergWittenDeformationTheory"
%%% End:

